Scaling Laws for Deep Learning

Running faster will only get you so far -- it is generally advisable to first understand where the roads lead, then get a car ... The renaissance of machine learning (ML) and deep learning (DL) over the last decade is accompanied by an unscalable computational cost, limiting its advancement and weighing on the field in practice. In this thesis we take a systematic approach to address the algorithmic and methodological limitations at the root of these costs. We first demonstrate that DL training and pruning are predictable and governed by scaling laws -- for state of the art models and tasks, spanning image classification and language modeling, as well as for state of the art model compression via iterative pruning. Predictability, via the establishment of these scaling laws, provides the path for principled design and trade-off reasoning, currently largely lacking in the field. We then continue to analyze the sources of the scaling laws, offering an approximation-theoretic view and showing through the exploration of a noiseless realizable case that DL is in fact dominated by error sources very far from the lower error limit. We conclude by building on the gained theoretical understanding of the scaling laws' origins. We present a conjectural path to eliminate one of the current dominant error sources -- through a data bandwidth limiting hypothesis and the introduction of Nyquist learners -- which can, in principle, reach the generalization error lower limit (e.g. 0 in the noiseless case), at finite dataset size.

==> Related.tex <==
\section{Related Work}
\label{sec:related}


\paragraph{Model scaling:}
A number of studies have explored the effect of model scaling on performance. 
For instance, image classification networks can be scaled by depth~\citep[number of layers;][]{he2016deep} or width~\citep[number of channels;][]{zagoruyko2016wide,howard2017mobilenets}. 
More recently, 
\citet{tan2019efficientnet} 
demonstrated how scaling width, depth, and input resolution has combined positive effects larger than  scaling each factor in isolation. Importantly, this method is inherently constructive.  However, a relationship between model scaling and error was yet to be quantified in a predictive form prior to this work -- e.g. by how much will error change with model scaling?
%In the absence of a principled approach towards model scaling, certain  heuristics have been found useful, such as exponentially increasing model size~\citep{radford2019language}. 
% In this work, we focus on finding a constructive functional form for determining the model given a specified performance. 

% \vspace{-5pt}
\paragraph{Data scaling:}
It has long been recognized that more data improves performance, and various studies report such trends in both computer vision~\citep[e.g.,][]{zhu2012we,sun2017revisiting} and language processing tasks~\citep[e.g.,][]{banko2001mitigating,talmor-berant-2019-multiqa}. 
A number of prior studies  observed power-law relations between the generalization error and training data size~\citep{cho2015much,miceli-barone-etal-2017-regularization,johnson-etal-2018-predicting}. 
Most relevant to our work, \citet{hestness2017deep}  explored the effect of data size on the generalization error in vision, language, and speech  tasks, and observed a strikingly consistent power-law behavior in a large set of experiments. However, while these studies point to the empirical \textit{existence} of a power law in terms of data, they are not constructive - i.e. they do not offer tools for  predicting the performance given a specified model.
Nor do they offer low-cost methods to specify the model configuration which would attain the power law with data dependency.
Indeed, \citeauthor{hestness2017deep}\ had to search over models and their configurations at large scale to exhibit their findings, incurring prohibitive computational costs.

In contrast, we demonstrate a constructive recipe, where we directly predict the test performance at large scale and specify the full model configuration which attains it (with no need for large-scale search), given performance at small scale. Importantly, our constructive framework deals jointly with the problem constituents of model size, degrees of freedom, sparsity and data size.

Following our work \ref{} perform a study on larger scale language models than in our work which corroborate our findings at that larger scale.

% \vspace{-5pt}
\paragraph{Predicting model performance:}
Since training models at full data/model scale may be computationally prohibitive, a line of work tries to predict the performance of a given model  on a given dataset, without training the model, for example by using a bank  of previously trained models, dataset, and their associated performances~\citep{istrate2019tapas}. However this line of work does not offer a functional form or means of reasoning about tradeoffs, nor does it work for de-novo tasks.

Others have proposed to forgo actual performance estimation, but rather estimate relative performance rank on small data~\citep{klein2017fast} or model sizes~\citep{zoph2018learning,real2019aging} in the context of neural architecture search (NAS). In this case, the small-scale evaluation is used to compare models at small cost, to expedite the search process; see~\cite{elsken2019neural} for a recent survey. 
However failure modes remain unclear and in particular circumstances needed for ranks to remain consistent across scales. 

Our work aims at a stronger requirement - namely, finding the error form itself from small scale measurments. As a special case, rank is predicted reliably, and need not be the same across scales. 

% \paragraph{Model sparsity and pruning}
% While achieving high performance has proven tantamount with training large models on large data, sparsity has emerged as a method reducing the number of parameters , and thus number of computations, needed for the evaluation of a new sample. Many different forms of inducing sparsity have been explored [add references here] including magnitude pruning, variational dropout and l0 regularization. Typically, the point of maximal sparsity such that little or no performance hit is incurred is of interest. In contrast, in this work we propose to push the sparsity levels as high as shy of network disconnection, in order to acertain if there what is the connection between the small model (high sparsity) and large model (low sparsity) errors.

% \vspace{-5pt}
\paragraph{Theoretical error bounds:}
Much attention has been given to theoretical explanations of the generalization capabilities of deep neural networks~\citep{%bartlett2017spectrally,
neyshabur2017exploring,neyshabur2017pac,allen2018learning,allen2018convergence,arora2018stronger}. While fully engaging with this literature is beyond our scope, we note that currently, to the best of our knowledge, no predictive framework exists explaining the generalization error exactly - i.e. giving a prediction rather than a loose upper bound and/or lower bound.

It is however interesting to further note that
% we note that %several 
recent studies have derived bounds involving power-law dependencies in both model~\citep{yarotsky2018optimal} and data size~\citep{liang2019risk}. We leave it as an open question for future work to find theoretical explanations for the empirical behavior and the functional form we investigate in this work. 

==> app4.tex <==
\chapter{Appendix A: Scaling Origins Additional Results and Implications}


\section{Investigation of the Deficiency Mechanism}

In Chapter \ref{sec:towards_origin} we have identified an optimization failure - Learning deficiency. In this section we further investigate its dependency, still in the realizable, noiseless case.

Since it is not noise which limits this mechanism, we consider how one may change the data-source. We thus explore two dimensions in which the data-generating teacher may be modified.


==> contributions.tex <==
\section{contributions}
\label{sec:contributions}

By completing this thesis, we expect to make the following contributions :

\begin{enumerate}
    \item Allow for a shift in NN research and development practices from (current) large scale to small scale in a principled manner
    \item Allow analytic and principled tradeoff design spanning issues as computational efficiency, constraint reasoning and early estimation of costs and expected results
    \item An an approximate, constructive prediction, of the error as function of model degrees of freedom and data. Thus in particular, we propose to provide a solution for optimal architectural configuration.
    % \item An an approximate, constructive prediction, of the error for sparse and dense models
    \item An empirical foundation for the search of the theoretical origins of the generalization error
\end{enumerate}




